Fully Dynamic All Pairs All Shortest Paths

We consider the all pairs all shortest paths (APASP) problem, which maintains all of the multiple shortest paths for every vertex pair in a directed graph $G=(V,E)$ with a positive real weight on each edge. We present two fully dynamic algorithms for this problem in which an update supports either weight increases or weight decreases on a subset of edges incident to a vertex. Our first algorithm runs in amortized $O({\nu^*}^2 \cdot \log^3 n)$ time per update, where $n = |V|$, and $\nu^*$ bounds the number of edges that lie on shortest paths through any single vertex. Our APASP algorithm leads to the same amortized bound for the fully dynamic computation of betweenness centrality (BC), which is a parameter widely used in the analysis of large complex networks. Our method is a generalization and a variant of the fully dynamic algorithm of Demetrescu and Italiano [DI04] for unique shortest path, and it builds on our recent decremental APASP [NPR14]. Our second (faster) algorithm reduces the amortized cost per operation by a logarithmic factor, and uses new data structures and techniques that are extensions of methods in a fully dynamic algorithm by Thorup.

==> Makefile <==
TEX = acmsmall-sample.tex \
	sample10.tex \
	sample11.tex \
	sample1.tex \
	sample2.tex \
	sample3.tex \
	sample4.tex \
	sample5.tex \
	sample6.tex \
	sample7.tex \
	sample8.tex \
	sample9.tex \


CLS = acmsmall.cls

STY = acmcopyright.sty

PACKAGE = acmsmall

PDF = ${TEX:%.tex=%.pdf} acm-update.pdf

PWD= ${shell pwd}

all: $(PDF)

%.pdf: %.tex $(CLS) $(STY)
	pdflatex $*
	bibtex $*
	pdflatex $*
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log)\
	do pdflatex $*; done

acm-update.pdf:  ../documentation/acm-update.tex
	cd ../documentation; ${MAKE}; cd ${PWD}; cp ../documentation/$@ .

acmcopyright.sty:  ../acmcopyright/acmcopyright.dtx
	cd ../acmcopyright; ${MAKE}; cd ${PWD}; cp ../acmcopyright/$@ .

clean:
	$(RM) *.aux *.log  *.blg

distclean: clean
	$(RM) $(PDF) acm-update.pdf *.bbl

zip: all clean
	zip $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

==> ffintro.tex <==
%\section{Introduction}
%
%Betweenness centrality (BC) is a widely-used measure
%in the analysis of large complex networks, and is defined as follows.
%Given a directed graph $G=(V,E)$ with $|V|=n$, $|E|=m$ and positive edge weights, let 
%$\sigma_{xy}$ denote the number of shortest paths (SPs)
%from $x$ to $y$ in $G$, and
%$\sigma_{xy}(v)$ the number of SPs from $x$ to $y$ in $G$ that pass through $v$, for each pair $x,y\in V$. 
%Then, $BC(v) = \sum_{s \neq v, t \neq v} \frac{\sigma_{st}(v)}{\sigma_{st}}$.
%As in \cite{Brandes01}, we assume positive edge weights to avoid the case when cycles of 0 weight are present in the graph. 
%
%The measure $BC(v)$  is often used as an index that  determines the relative importance of
%$v$ in $G$, and is computed for all $v\in V$.
%Some applications of
%BC include analyzing social interaction networks \cite{KA12},
%identifying lethality in biological networks \cite{PCW05},
%and identifying key actors in terrorist networks \cite{Coffman,Krebs02}.
%In the static case,
%the widely used algorithm by Brandes~\cite{Brandes01} runs in 
%$O(mn + n^2 \log n)$ on weighted graphs.
%Several approximation algorithms are available: \cite{BaderKMM07,Riondato} for static computation and, recently, \cite{Bergamini1,Bergamini2} for dynamic computation.
%Heuristics for dynamic betweenness centrality with good experimental
%performance are given in~\cite{GreenMB12,Lee12,SinghGIS13},
%but none provably improve on Brandes.
%The only earlier exact  dynamic BC algorithms that provably improve on
%Brandes on
%some classes of graphs are the recent separate incremental and decremental\footnote{Incremental/decremental 
%	refer to the insertion/deletion of a
%	vertex or edge; the corresponding weight changes that apply are 
%	weight decreases/increases, respectively.}
%algorithms in~\cite{NPR14,NPR14b}. Recently, we give in \cite{PR14} (see also \cite{PR15i}) the first fully dynamic algorithm for BC (the \PR method) that is provably faster than  
%Brandes for the class of dense graphs 
%(where $m$ is close to $n^2$)
%with succinct single-source SP dags.
%Table~\ref{table1} contains a summary of these results.
%
%In this paper, we present an improved algorithm for computing fully dynamic exact betweenness centrality: 
%our algorithm \FFD 
%improves over \PR by a logarithmic factor
%using data structures and technique that are considerably more complicated.
%Our method is a generalization of
%Thorup~\cite{Thorup04} (the \Tho method) which computes fully dynamic APSP
% for graphs with a unique SP for every vertex pair; however, a key step in BC algorithms is computig  \emph{all} SPs for each pair of vertices (\emph{all pairs 
% \underline{all} shortest paths --- AP\underline{A}SP}).    We develop a faster fully dynamic algorithm for APASP, which in turn 
%  leads to a faster fully dynamic BC algorithm than \PRe.

\vone
\noindent
{\bf Our Results.} 
Let $\vstar$ be the maximum
number of distinct edges that lie on shortest paths through any given vertex in $G$; 
for convenience we assume $\nu^* = \Omega (n)$.





\noindent
{\bf Discussion of the parameters $m^*$ and $\vstar$.}
Let $m^*$ be the number of distinct edges in $G$ that lie on shortest paths; $\nu^*$, defined above, is the maximum number of distinct
edges on any single source SP dag. Clearly, $\nu^* \leq m^* \leq m$.\\
- \underline{$m^* \textrm{ vs } m$}: In many cases,  $m^* \ll m$:
	as noted in \cite{KKP93}, in a complete graph ($m=\Theta(n^2$)) where edge weights are chosen from
	a large class of probability distributions, $m^* = O(n \log{n})$
	with high probability. 
	
	\vhalf
	\noindent
- \underline{$\vstar \textrm{ vs } m^*$}: Clearly, $\vstar =O(n)$ in any graph with only a constant number of SPs between every
	pair of vertices. These graphs are called $k$-geodetic \cite{kgeo} (when at most $k$ SPs exists between two nodes), and are well studied in graph theory \cite{bigeo,bandelt,mulder}.
In fact $\vstar = O(n)$ even in some graphs that have an exponential number of SPs between some pairs of vertices.

    In contrast, $m^*$ can be $\Theta (n^2)$  even in some graphs with unique SPs, for example the complete unweighted
    graph $K_n$.
    
    Another type of graph with  $\vstar \ll m^*$ is one with large clusters of nodes
    (e.g., as described by the \emph{planted $\ell$-partition model} \cite{Condon,clusters}).
    Consider a graph $H$ with $k$ clusters of size  $n/k$ (for some constant $k \geq 1$) with
    $\delta < w(e) \leq 2\delta$, for some constant $\delta>0$,  for each edge $e$ in a cluster;
    between the clusters is a sparse
    interconnect. Then
    $m^* = \Omega(n^2)$ but $\vstar= O(n)$. (The  connections between clusters can be arbitrary, thus  BC scores are non-trivial to compute.)
    For all of the above classes of graphs, our BC algorithm
    will run in amortized $\tilde O(n^2)$ 
    time per update ($\tilde O$ hides polylog factors). More generally we have:
    


Our algorithm uses $\widetilde{O}(m \cdot \vstar)$ space, extending the $\widetilde{O}(mn)$ 
result
in \DI for APSP. Brandes uses only linear space, but all
known
dynamic algorithms require at least 
$\Omega (n^2)$ space.
	
\vhalf
\noindent
{\bf Overview of the Paper.} 
In Section \ref{sec:fdbc} we describe how to obtain a fully dynamic BC algorithm using a fully dynamic  APASP algorithm. The remaining
sections in the paper are devoted to developing our improved fully dynamic APASP algorithm.
In Section \ref{sec:bkg} we review the \NPRe and \PR and \Tho methods. 
In Section \ref{subsec:fully-impl} we introduce the level \system framework for APASP, with particular reference to  the new data structures specifically developed for our result.
In Section~\ref{sec:algo} we  present our algorithm \FFDe, and we describe its main components in detail.
Section \ref{sec:ffeatures} describes two important challenges that arise when generalizing \Tho to APASP setting; addressing these two challenges is crucial to the correctness and efficiency of our algorithm. 
Finally, in Section \ref{sec:proof} we establish the  amortized time bound of $O({\nu^*}^2 \cdot \log^2 n)$ for \FFD and its correctness. 

==> repres-trimmed.tex <==
\vspace{-0.1in}
\subsubsection{A System of Tuples}
\label{sec:tuple-system}

VLR: To be trimmed further

 We present succinct representations for sets of SPs and LSPs in the
 edge-weighted graph $G=(V,E)$ using the notions of {\em tuple} and {\em triple}.


\noindent
{\bf Tuple.}
A tuple, $\tau = (xa, by)$, represents the set of LSPs in $G$, all 
of which  use
the same first edge $(x,a)$ and the same last edge $(b,y)$. 
The weight of every path
represented by $\tau$ is $\weight(x, a)$ + $d(a, b) + \weight(b,y)$. 
We call $\tau$ a {\it locally shortest path tuple (LST)}.
In addition, if $d(x, y) = \weight(x, a) + d(a, b) + \weight(b, y)$, then 
$\tau$ is a {\it shortest path tuple (ST)}.


\noindent
{\bf Triple.}
A triple $\gamma=(\tau, wt, count)$, represents the tuple $\tau=(xa,by)$ that contains
$count$ number of paths from $x$ to $y$, each with weight
$wt$. In Fig.~\ref{fig:illust-example}, the triple $((xa_2,by),4,2)$ represent two paths of weight $4$ from $x$ to $y$.
%MN: June 24, 2014. Added the explicit paths since this is the first time.
%namely $p_1 = \langle x, a_2, v, b, y \rangle$ and $p_2 = \langle x, a_2, v_2, b, y \rangle$.

\vone
\noindent
{\bf Storing Locally Shortest Paths.}
\label{sec:storing-LST}
We use triples to succinctly store 
%VLR
all
%
LSPs and SPs
for each vertex pair
%
 in $G$. For $x, y \in V$,
 %VLR
 we define:
%
\begin{eqnarray*}
P(x,y) &=& \{\mbox{$((xa, by), wt, count)$: $(xa, by)$ is an LST from $x$ to $y$ in $G$} \} \\
P^{*}(x,y) &=& \{\mbox{$((xa, by), wt, count)$: $(xa, by)$ is an ST from $x$ to $y$ in $G$} \}.
\end{eqnarray*}
 Note that all triples in $P^{*}(x,y)$ have the same weight.  We use the term LST to denote locally shortest triples as well
as tuples 
and it will be clear from the context whether we mean a triple or a tuple.

\vone
\noindent
{\bf Left Tuple and Right Tuple.}
%
A left tuple (or $\ell$-tuple), 
$\tau_{\ell} = (xa, y)$,
represents the
set of LSPs from $x$ to $y$, all of which use 
the same first edge $(x,a)$.
The weight of every path
represented by $\tau_{\ell}$ is $\weight(x, a)$ + $d(a, y)$.
If $d(x, y) = \weight(x, a) + d(a, y)$, then $\tau_{\ell}$ represents the
set of shortest paths from $x$ to $y$,
all of which use the first edge $(x, a)$. 
A right tuple ($r$-tuple) $\tau_r = (x, by)$ is defined analogously.
% 
In the following, we will say that a tuple (or $\ell$-tuple or $r$-tuple)
{\it contains} a vertex $v$, if at least one of the paths represented by the
tuple contains $v$.

\vone
\noindent
{\bf ST and LST Extensions.}
%
For a shortest path $r$-tuple $\tau_r = (x, by)$, we
define $L({\tau_r})$ as
the set of vertices which can be used as pre-extensions to create  LSTs
in~$G$.
Similarly, for a shortest path $\ell$-tuple $\tau_{\ell} = (xa, y)$,
$R(\tau_{\ell})$ is the set of vertices which can be used as post-extensions to
create LSTs in $G$. We do not 
define $R(\tau_r)$ and $L(\tau_{\ell})$. 
So we have:
\begin{eqnarray*}
L(x, by) &=& \{x': \mbox {$(x', x) \in E(G)$ and $(x'x, by)$ is an LST in $G$}\} \\
R(xa, y) &=& \{y': \mbox {$(y, y') \in E(G)$ and $(xa, yy')$ is an LST in $G$}\}.
\end{eqnarray*}

For $x, y \in V$, $L^{*}(x, y)$ denotes the set of vertices which can 
be used as pre-extensions to create shortest path tuples in $G$;
$R^{*}(x, y)$ is defined symmetrically:
\begin{eqnarray*}
L^{*}(x, y) &=& \{x': \mbox {$(x', x) \in E(G)$ and $(x'x, y)$ is a $r$-tuple representing SPs in $G$}\} \\
R^{*}(x, y) &=& \{y': \mbox {$(y, y') \in E(G)$ and $(x, yy')$ is an $\ell$-tuple representing SPs in $G$}\}.
\end{eqnarray*}

\vspace{-0.12in}
\paragraph{\bf Key Deviations from DI \cite{DI04}.} 
The assumption of unique shortest paths in \cite{DI04} 
ensures that $\tau = (xa, by)$,
$\tau_{\ell} = (xa, y)$, and $\tau_r = (x, by)$ all represent exactly the
same (single)  locally shortest path.
However, in our case, the set of paths represented by 
$\tau_{\ell}$ and $\tau_r$ can be different, and 
$\tau$ is a subset of paths represented by $\tau_{\ell}$ and
$\tau_r$. 
Our definitions of ST and LST extensions are
derived from the analogous definitions in \cite{DI04} for SP and LSP
extensions of paths.
For a path $\pi = x \rightarrow a \leadsto b \rightarrow y$,
DI defines sets $L$, $L^{*}$, $R$ and $R^{*}$.
In our case,
 the analog of a path $\pi = x \rightarrow a \leadsto b \rightarrow y$ 
is a tuple $\tau = (xa, by)$, 
but to obtain efficiency, we  define
the set $L$ only for an $r$-tuple and the set $R$ only for an $\ell$-tuple. 
Furthermore, we define  $L^{*}$ and $R^{*}$ for each
pair of vertices. 


\begin{lemma}
\label{lem:total-locally-shortest}
\cite{NPR14b}
The number of LSTs (or triples) in $G=(V,E)$ is bounded by $O(m^* \cdot \vstar)$.
\end{lemma}

\begin{lemma}
\label{lem:bound-tuples-thru-v}
\cite{NPR14b}
The number of LSTs (or triples) that contain a vertex $v$  
is $O({\vstar}^2)$.
\end{lemma}


